Data-Efficient Contrastive Self-supervised Learning: Most Beneficial Examples for Supervised Learning Contribute the Least

Self-supervised learning (SSL) learns high-quality representations from large pools of unlabeled training data. As datasets grow larger, it becomes crucial to identify the examples that contribute the most to learning such representations. This enables efficient SSL by reducing the volume of data required. Nevertheless, quantifying the value of examples for SSL has remained an open question. In this work, we address this problem for the first time, by proving that examples that contribute the most to contrastive SSL are those that have the most similar augmentations to other examples, in expectation. We provide rigorous guarantees for the generalization performance of contrastive learning on such subsets. Through extensive experiments, we show that we can safely exclude 20% of examples from CIFAR100 and 40% from STL10 and TinyImageNet, without affecting downstream task performance. In general, subsets selected by our method outperform random subsets by over 3% across these datasets. Interestingly, we also discover the subsets that contribute the most to contrastive learning are those that contribute the least to supervised learning. Code available at https://github.com/bigml-cs-ucla/sas-data-efficient-contrastive-learning.

==> method-old.tex <==
\section{The Most Essential Subset for SSL}
\sj{fix $f_S$ and $f$} To address the above problem, we aim to find
% Our goal is to select 
a subset of unlabeled training examples $S\subseteq V$, such that minimizing the contrastive loss in Eq. \eqref{eq:cl_loss} on the subset $S$ results in a similar encoder $f^S$ to the encoder $f$ obtained by minimizing the contrastive loss on the full data $V$. This ensures learning similar representations for all the training examples, and consequently a superior generalization performance for the NN classifier. 

% \ba{fix:} Formally, our goal is to find a subset $S_k$ of size at most $r_k$ from every latent class $V_k$, such that minimizing the alignment loss on the union of subsets $S=\cup_k S_k$ results in an encoder $f^S$ which minimizes $R_{\epsilon}(f^S,V)$ on the entire data. Formally: \ba{change to trained network}
% \begin{align}\label{problem:align}
%    \hspace{-1mm}S^*\!\!\in\hspace{-4mm}\argmin_{ \substack{S=\cup_{k\in [K]} S_k,\\ S_k\subseteq V_k,|S_k|\leq r_k}} \!\!\!\!\!\!\LL_{cl}(f^S\!,\!V)~~ \text{s.t.}~
%     &f^S\!\!=\!\argmin_f \LL_{cl}(f,S), %\nonumber
% \end{align}

\subsection{Motivation: Generalization of SSL Representations}
To find such a subset, we rely on recent results on providing generalization guarantees for contrastive learning. In particular, the very recent results of \citet{huang2021towards} showed that the generalization performance of a model trained with contrastive learning %can be upper-bounded by
is \sj{dependent on?} related to the (1) alignment of positive samples, (2) divergence of class centers, and (3) concentration of the augmented data.
% , i.e., small $\min_{\x_1,\x_2\in A(\x)}\norm{\x_1-\x_2}$ for the majority of examples (the main part) in every class. 
%%%
Alignment is defined as  $\E_{i\in V}\E_{\x_1,\x_2\in A(\x_i)}\norm{f(\x_1)-(\x_2)}^2$, and good alignment requires augmented views of each example to have similar representations, in expectation. \sj{rephrase?} Divergence \sj{of class centers} is captured by $\muu_l^T\muu_k$, good divergence results in large enough distance between class centers (small $\muu_l^T\muu_k$).
Finally, the data has a sharp augmentation concentration if the majority of examples (the main part) in every class, %have a %small augmented distance
% sharp concentration of augmented data, i.e., 
have a similar augmented view \sj{rephrase?}, i.e.,
$\sup_{\x_1,\x_2} \min_{\x'_1\in A(\x_1),\x'_2\in A(\x_2)}\norm{\x_1-\x_2}\leq \delta$.

%%%%%%%%%%%%%%%%%%%%%
% Effectively, minimizing the contrastive loss results in minimizing the alignment, and yields a good divergence between centers of examples in the main part of every class.
Formally, for a normalized encoder $\norm{f}=1$, the InfoNCE loss in Eq. \eqref{eq:cl_loss} can be written as:
\begin{align}\label{eq:loss_equiv}
    \LL_{cl}(&V)
    \!=\!\frac{1}{2}[\E_{i\in V}\E_{\x_1,\x_2\in A(\x_i)}\!\norm{f(\x_1)\!-\!f(\x_2)}^2]\!-\!1\\
    &+\!\!\!\!\E_{i,j\in V} \;\E_{\substack{\x_1,\x_2\in A(\x_i)\\ \x^-\!\in A(\x_j)}}\log(e^{f(\x_1)^Tf(\x_2)}+e^{f(\x_1)^Tf(\x^-)})\nonumber
\end{align}
The first term in the RHS of Eq. \eqref{eq:loss_equiv} is closely related to the alignment and the second term is related to divergence. %More precisely, the recent result of \cite{huang2021towards} showed that minimizing the contrastive loss directly minimizes the alignment, and also minimizes as an upper-bound on the divergence $\muu_l\muu_k$. 
%%%%%%%%%%%%%%%%%%%%
At a high level, if the majority of examples (the main part) in every class have a sharp concentration of augmented data, then minimizing the contrastive loss results in an encoder with 
good alignment, %i.e., small $\E_{\x}\E_{\x_1,\x_2\in A(\x)}\norm{f(\x_1)-(\x_2)}^2$, 
and good divergence.
% , i.e., large enough distance between class centers (small $\muu_l^T \muu_k$).
With good alignment and divergence, the NN classifier $g_f$ can correctly classifies all the examples in the main part of every class with aligned augmented views. %, and achieves a superior generalization guarantee.
If the main part of every class is sufficiently large, a superior \sj{rephrase?} generalization performance is guaranteed. 

\subsection{Towards Finding Generalize Subsets}
The key idea of our approach is to find a subset such that training on it (1) results in a small alignment for all the examples in every class, and (2) preserves the class centers. If such a subset can be found, minimizing the contrastive loss in Eq. \eqref{eq:cl_loss} on the subset results in an encoder with good alignment and divergence on the entire training data, and guarantees a similar generalization performance for the downstream NN classifier. \looseness=-1
% This implies that a subset that provides similar generalization guarantees to that of full data for contrastive SSL, should yield (1) high alignment for sharply-concentrated examples of each class and (2) preserves the class centers. 

Next, we introduce the notion of expected augmentation distance, and discuss how it can be leveraged to find a subset that satisfies the above two conditions.

\begin{definition}[\textbf{Expected augmentation distance}]
We define the expected augmentation distance between examples $i,j\in V$ as the expected $l_2$ norm between \sj{\textbf{representations}} of augmented views of $\x_i, \x_j$, i.e. $A(\x_i)$, $A(\x_j)$. Formally, for every pair of examples $i,j\in V$ we have: %\ba{over time?}
\begin{equation}\label{eq:dist}
    d_{i,j}=\E_{\substack{\x\in A(\x_i),\\\x'\in A(\x_j)}} \|\rf{\x} - \rf{\x'}\|.
\end{equation}
\end{definition}
Intuitively, expected augmentation distance captures the semantic similarity between examples. \sj{more?} Effectively, $d_{i,j}$ is small if augmented views of $\x_i$ and $\x_j$ have similar representations, in expectation.  
% Hence, the expected augmentation distance between examples in different latent classes is 0, as they are not semantically similar. \ba{relax this?}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth, keepaspectratio]{Fig/exp_aug_dist.png}
    \vspace{-8mm}
    \caption{Expected augmentation distance $d_{i,j}$ is small for examples $\x_i,\x_j$ which have similar augmentations.}
    \label{fig:cifar10}
\end{figure}
%%%%%%%%%%%%%%%
\subsection{Ensuring Good Alignment}
We start by finding a subset that when used to minimize the contrastive loss, provides a good alignment for all the training examples. 
%%%%%%%%%%%%%%%
Note that minimizing the alignment loss: \begin{equation}
\!\LL_{align}(V)\!=\!\E_{i\in V}\! \E_{\x_1,\x_2\in A(\x_i)}\!\|f(\x_1)\!-\!f(\x_2)\|^2
\end{equation} 
directly minimizes the probability $R_{\epsilon}(f,V) $ of examples that have non-aligned augmented views, i.e, the largest distance between their augmented views is larger than $\epsilon$: \looseness=-1
\begin{equation}
    R_{\epsilon}(V) = \mathbb{P} \Big[ i\in V: \!\!\!\!\!\!\sup_{\x_1,\x_2\in A(\x_i)} \!\!\!\!\|f(\x_1)-f(\x_2)\|>\epsilon \Big]. 
\end{equation}
In fact, for a $L$-Lipschitz continuous encoder $f$, we have that \cite{huang2021towards}: %minimizing the contrastive loss in Eq. \!\eqref{eq:cl_loss} directly minimizes $R_{\epsilon}\!$ . I.e.,
\begin{align} \vspace{-3mm}
    R_{\epsilon}(V)\leq \eta(\epsilon)\!\cdot\!\sqrt{\LL_{align}(V)},
\end{align}
where $\!\eta(\epsilon)\!=\!\mathcal{O}(\frac{1}{\epsilon})\!$ is a function of $\epsilon$ and the transformations used for data augmentations.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Formally, we wish to solve the following bilevel optimization problem:\looseness=-1
% \begin{align}\label{problem:align}
%    \hspace{-2mm}S^*\in\!\!\argmin_{ \substack{S=\cup_{k\in [K]} S_k,\\ S_k\subseteq V_k,|S_k|\leq r_k}} \!\!&R_{\epsilon}(f^S,V)~~ \text{s.t.}~~\\
%     &f^S=\argmin_f \LL_{align}(f,\cup_{k\in[K]} S_k), \nonumber
% \end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% when used to minimizing the contrastive loss provides a good alignment for the entire training data.
% First, we show that a subset with a small expected augmentation distance to other examples in class $k$ ensures a small alignment for all the examples in the class. Formally, alignment is defined as follows:
% where $\!\LL_{align}(f,S)\!=\!\E_{i\in S}\! \E_{\x_1,\x_2\in A(\x_i)}\!\|f(\x_1)\!-\!f(\x_2)\|^2$. \looseness=-1



% Let $R_{\epsilon}$ be the probability of examples that do not have a good alignment. That is, the largest distance between their augmented views is larger than $\epsilon$:

% Therefore, our goal is to find a subset such that minimizing the contrastive loss on the subset minimizes $R_{\epsilon}$ on the entire dataset.
For every (arbitrary) subset $S_k\subseteq V_k$ of size $r_k=|S_k|$ selected from class $k$ with $n_k=|V_k|$ examples, we can upper-bound the probability $R_{\epsilon}(V_k)$ for all examples in the class, based on the alignment of the subset calculated using the same encoder $\LL_{align}(S_k)$:  
\begin{align}
    &R_{\epsilon}(V_k)\leq \eta(\epsilon)\cdot\sqrt{\LL_{align}(V_k)}\\
    &\!= \eta(\epsilon) \!\cdot\! \Big(\E_{i\in V_k}\E_{\x_1,\x_2\in A(\x_i)} \|f(\x_1)-f(\x_2)\|\Big)\\
    &\!= \frac{\eta(\epsilon)}{n_k} \!\cdot\! \Bigg( \sum_{i \in S_k}\E_{\x_1,\x_2\in A(\x_i)} \norm{f(\x_1)-f(\x_2)} \\
    &\hspace{2cm} + \sum_{j \in V_k\setminus S_k}\E_{\x_1,\x_2\in A(\x_j)} \norm{f(\x_1)-f(\x_2)} \!\Bigg) \nonumber\\
    &\!\leq \frac{\eta(\epsilon)}{n_k} \!\cdot\! \Bigg(\!{r_k}\sqrt{\LL_{align}(S_k)} +\!\!\!\!\!\sum_{i\in V_k\setminus S_k}\!\!\! [\min_{j\in S_k} d_{i,j}\!+\epsilon']\!\Bigg), 
    % &\hspace{2cm} + \sum_{j \in V_k\setminus S_k} \max_{\substack{\x_1,\x_2\in A(\x_i)}} \norm{f(\x_1)-f(\x_2)} \Bigg) \nonumber\\
    % &\!\leq \frac{\eta(\epsilon)}{n_k} \!\cdot\! \Bigg({r_k}\sqrt{\LL_{align}(f,S_k)} \\
    % &\hspace{2cm} + \sum_{j \in V_k\setminus S_k} \max_{\substack{\x_1,\x_2\in A(\x_i)}} \norm{f(\x_1)-f(\x_2)} \Bigg) \nonumber\\
\end{align}    
% \begin{align}
%     d_{i,j}=\!\!\!\E_{\x,\x'\in A(\x_i)}\!\!\!\norm{f(\x)-f(\x')}\leq n_{a} \!\!\!\max_{\x,\x'\in A(\x_i)}\!\!\!\norm{f(\x)-f(\x')} \nonumber
% \end{align}
%%%%%%%%%%%%%%%%% previous %%%%%%%%%%%%
% \begin{align}\label{eq:r_errorr}
%     &R_{\epsilon}(f^{},V_k)\leq \eta(\epsilon)\cdot\sqrt{\LL_{align}(f,V_k)}\\
%     &\!= \eta(\epsilon) \!\cdot\! \Big(\E_{i\in V_k}\E_{\x_1,\x_2\in A(\x_i)} \|f(\x_1)-f(\x_2)\|\Big)\\
%     &\!= \frac{\eta(\epsilon)}{n_k} \!\cdot\! \Bigg( \sum_{i \in S_k}\E_{\x_1,\x_2\in A(\x_i)} \norm{f(\x_1)-f(\x_2)} \\
%     &\hspace{2cm} + \sum_{j \in V_k\setminus S_k}\E_{\x_1,\x_2\in A(\x_j)} \norm{f(\x_1)-f(\x_2)} \!\Bigg) \nonumber\\
%     % &\!\leq \eta(\epsilon) \cdot \left(\frac{r_k}{n_k} \sqrt{\E_{\x \in S}\E_{\x_1,\x_2\in A(\x)} \norm{f(\x_1)-f(\x_2)}^2} + \left(1 - \frac{r_k}{n_k} \right) \E_{\x' \notin S}\E_{\x_1,\x_2\in A(\x')} \norm{f(\x_1)-f(\x_2)} \right) \\
%     &\!\leq \frac{\eta(\epsilon)}{n_k} \!\cdot\! \Bigg({r_k}\sqrt{\LL_{align}(f,S_k)} +  \\
%     &\hspace{2.4cm} ~~~ \sum_{j\in V_k\setminus S_k}\E_{\x_1,\x_2\in A(\x_j)} \norm{f(\x_1)-f(\x_2)} \!\!\Bigg) \nonumber\\
%     % &\!\leq \eta(\epsilon) \cdot \left(\frac{r_k}{n_k} \sqrt{\LL_{align}(f^S)} + \left(1 - \frac{r_k}{n_k} \right) \E_{\x' \notin S}\Big[\E_{\x \in S}\big(\E_{\x_1,\x_2\in A(\x)}\norm{f(\x_1)-f(\x_2)}+%\E_{\x\in S} 
%     % d_{\x,\x'}\big)\Big] \right) \\
%     &\!\leq \frac{\eta(\epsilon)}{n_k} \!\cdot\! \Bigg( r_k \sqrt{\LL_{align}(f,S_k)}  + (n_k-r_k)  \\
%     &\hspace{2cm}~~~\sqrt{\LL_{align}(f,S_k)}+ \frac{1}{r_k}\sum_{j \in V_k\setminus S_k}\sum_{i \in S} d_{i,j} \Bigg) \nonumber\\
%     &=\eta(\epsilon) \!\cdot\!\Bigg(\! \sqrt{\LL_{align}(f,S_k)}\!+\!  \frac{1}{n_k r_k}\sum_{j\in V_k\setminus S_k}\sum_{i \in S_k} d_{i,j} \Bigg)\nonumber
%     % &=\eta(\epsilon) \cdot\left( \sqrt{\LL_{align}(f^S)}+  \left(1 - \frac{r_k}{n_k} \right)\left(\frac{n_k}{n_k-r_k}\E_{\x' \in C_k}\E_{\x \in S} d_{\x\x'} - \frac{r_k}{n_k-r_k}\E_{\x' \in S_k}\E_{\x \in S} d_{\x\x'}  \right)\right)\\
%     % &=\!\eta(\epsilon) \!\cdot\!\!\Big( \!\sqrt{\LL_{align}(f^S)}+ \!\!\!\!\E_{\substack{\x'\in V_k,\\ \x \in S_k}} \![d_{\x,\x'}] \!- \!\frac{r_k}{n_k} \!\E_{\substack{\x,\x' \in S_k}} \![d_{\x,\x'}] \Big).\nonumber
% \end{align}
% \begin{lemma}\label{lemma:align}
% If encoder $f$ is $L$-Lipschitz continuous, then training on a subset $S$ results in the following upper-bound on $R_{\epsilon}$ for all the examples $V_k$ in class $k$:
%     \begin{align}
%         R_{\epsilon}\!\leq\!\eta(\epsilon) \!\cdot\!\!\Big( \!\sqrt{\LL_{align}(f^S)}+ \!\!\!\!\E_{\substack{\x'\in V_k,\\ \x \in S_k}} \![d_{\x,\x'}] \!- \!\frac{r_k}{n_k} \!\E_{\substack{\x,\x' \in S_k}} \![d_{\x,\x'}] \Big).\nonumber
%     \end{align}
%%%%%%%%%%%%%%%%% previous %%%%%%%%%%%%
% \end{lemma}
% Lemma \ref{lemma:align} shows
% Minimizing the contrastive loss in Eq. \eqref{eq:cl_loss} ensures good alignment for the examples in the subset. Hence, $\LL_{align}(f^S)$ is small.
% Therefore, we get that
% \begin{equation}
%     \min_{S_k\subseteq V_k} R_{\epsilon}(f,V_k) \leq \min 
% \end{equation}
where $\epsilon'=\max_{j\in S_k,\x,\x'\in A(\x_j)}\norm{f(\x)-f(\x')}$ is the largest distance between augmented views of every examples $j\in S_k$. 
In particular, as $\LL_{align}(S_k)$ and $\LL_{align}(V_k)$ can both be effectively minimized (in Appendix we show that $\LL_{align}(S_k)$ is smaller on the subset, compared to random subsets of the same size, and to the full data \ba{show}), the subset introduces the following error on $R_{\epsilon}(V_k)$:
\begin{equation}\label{eq:r_error}
    \nu_R^k=|R_{\epsilon}(V_k)\!-\! R^S_{\epsilon}(V_k)|\!\leq \!\eta(\epsilon)\!\cdot\!\frac{r_k}{n_k}\!\!\!\sum_{i\in V_k\setminus S_k}\!\!\! [\min_{j\in S_k} d_{i,j}\!+\epsilon'],
\end{equation}
where $R^S_{\epsilon}(V_k)$ is the probability that an example in $V_k$ has a distance larger than $\epsilon$ between its augmented views, when minimizing $\LL_{align}(S_k)$.
We see that minimizing the alignment on the subset $S_k$ minimizes the alignment $\LL_{align}(V_k)$ and hence $R_{\epsilon}(V_k)$ on the entire class, with an error that is proportional to the expected augmentation distance between every example $i\in V_k\setminus S_k$ and data point $j\in S$ with the smallest augmentation distance.
Note that minimizing the alignment on $S_k$ results in a small $\epsilon$.
% examples in the subset $S_k$ and the rest of examples $V_k\setminus S_k$ in the latent class $k$. \ba{alignment loss can be minimized on all subsets to the same extent?}
% minimizes the probability $R_{\epsilon}(f,V_k)$ for all the examples in the class. 
Intuitively, a subset with small expected augmentation distance to the rest of the examples in the class includes examples that are semantically similar to all the examples in the class. \ba{can write error}
% \ba{subset alignment loss is at most alignment loss on V?}
% by ensuring that every example in the main part of the class is close to the subset. 
% Therefore, if augmentations are mostly concentrated about their expectation, SSL on the subset also ensures good alignment for other example in the main part of the class. 
% In addition, it shows the motivation for the examples in the subset to not be similar to each other. \ba{Todo: confirm}

% On the other hand, finding a subset by solving the minimization Problem \eqref{eq:subset} ensures that every example in the sharply concentrated part of the class is close to the subset. 

\subsection{Preserving the Class Centers}
Next, we discuss finding a subset that captures the center of every latent class $\muu_k$. 

For every (arbitrary) subset $S_k\subseteq V_k$ of size $r_k=|S_k|$ selected from class $k$ with $n_k=|V_k|$ examples, we can write the class center as follows:
% \begin{align}
%     \muu_k &= \E_{\substack{\x\in V_k,\\ \x'\in A(\x)}} \rf{\x'}\\
%     &=\E_{\substack{\x\in V_k,\\ \x'\in A(\x)}}\!\!\! \rf{\x'}\;-\E_{\substack{\x\in S_k,\\ \x'\in A(\x)}}\!\!\! \rf{\x'}\;+\E_{\substack{\x\in S_k,\\ \x'\in A(\x)}}\!\!\! \rf{\x'}\\
%     &=\frac{1}{|A(V_k)|} \sum_{\x'\in A(V_k)} \rf{x'} - \frac{1}{|A(S_k)|} \sum_{\x'\in A(V_k)} \rf{\x'} + \muu_k^S\\
%     &=\frac{1}{|A(V_k)|\cdot |A(S_k)|} [|A(S_k)|\sum_{\x'\in A(V_k)} \rf{\x'} - |A(V_k)|\sum_{\x\in A(S_k)} \rf{\x''}]-\muu_k^S\\
%     &=\frac{1}{|A(V_k)|\cdot |A(S_k)|} \sum_{\x'\in A(V_k)} \sum_{\x'\in A(S_k)} (\rf{\x'}-\rf{\x''})-\muu_k^S\\
%     &=\E_{\x'\in A(V_k)} \E_{x'\in A(S_k)} (\rf{\x'}-\rf{\x''})-\muu_k^S
% \end{align}
\begin{align}
    \muu_k \!&= \E_{\substack{\i\in V_k, \\ \x'\in A(\x_i)}} [\rf{\x'}] \nonumber\\
    &\!\!\!=\E_{\substack{i\in V_k,\\ \x'\in A(\x_i)}}\!\!\! [\rf{\x'}]\;-\E_{\substack{j\in S_k,\\ \x''\in A(\x_j)}}\!\!\! [\rf{\x''}]\;+\E_{\substack{j\in S_k,\\ \x''\in A(\x_j)}}\!\!\! [\rf{\x''}] \nonumber\\
    &\!\!\!=\frac{1}{n_k}\!\sum_{i\in V_k} \!\!\E_{\x'\in A(\x_i)} [\rf{\x'}] \!-\! \frac{1}{r_k}\!\sum_{j\in S_k} \!\!\E_{\x''\in A(\x_j)} [\rf{\x''}] + \muu_k^S \nonumber\\
    &\!\!\!=\!\!\frac{1}{n_k\!\cdot \!r_k} \Big[r_k\!\!\sum_{i\in V_k}\!\!\E_{\x'\!\in\! A(\x_i)}\!\!\!\! [\rf{\x'}] \!-\! n_k\!\!\sum_{j\in S_k}\!\!\E_{\x''\!\in \!A(\x_j)}\!\!\!\! [\rf{\x''}]\Big]\!+\!\muu_k^S \nonumber\\
    &\!\!\!=\!\frac{1}{n_k\!\cdot \!r_k} \!\sum_{i\in V_k} \!\sum_{j\in S_k} \!\!\big[\E_{\x'\!\in\! A(\x_i)}[\rf{\x'}]-\!\!\!\!\!\!\E_{\x''\!\in\! A(\x_j)}\![\rf{\x''}]\big]\!+\!\muu_k^S \nonumber\\
    &\!\!\!=\frac{1}{n_k\!\cdot \!r_k} \sum_{i\in V_k} \sum_{\j\in S_k} \! \E_{\substack{\x'\in A(\x_i),\\ \x''\in A(\x_j)}}\![\rf{\x'}\!-\!\rf{\x''}] +\muu_k^S %\nonumber\\
    % &=\frac{1}{n_k\!\cdot \!r_k} \sum_{\x\in V_k} \sum_{\x'\in S_k} d_{\x',\x''}+\muu_k^S 
\end{align}
Hence, we can upper-bound the normed difference between the center of class $V_k$ and subset $S_k$ as follows:
\begin{align}\label{eq:mu_error}
    \nu_{\mu}^k=\|\muu_k-\muu_k^S\|\!\leq %\frac{1}{n_k\!\cdot \!r_k}\!\! \sum_{\x'\in V_k} \sum_{\x'\in S_k}d_{\x,\x'}=
    \!\!\E_{\substack{i\in V_k,\\ j \in S_k}}[d_{i,j}]. %=\!\!\!\!\E_{\substack{i\in V_k\setminus S_k,\\ j\in S_k}}[d_{i,j}]+\!\!\E_{\substack{i,j\in S_k}}[d_{i,j}].
\end{align}
That is, the subset that preserves the center of class $k$, can be found by minimizing the expectation of expected augmentation distances between examples in the subset $S_k$ and all the data points $V_k$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Eq. \eqref{eq:r_error} and \eqref{eq:mu_error} show that the subset that closely captures the center of class $k$ and the ensures a small alignment on all data points in the class can be obtained by minimizing the expected augmentation distance between the subset and all examples in the class, condition on every example in the class is close enough in augmentation distance to an element in the subset, which encourages diversity in the subset: 
\begin{equation}\label{eq:subset}
    S_k^*=\!\!\!\!\argmin_{\substack{S\subseteq V_k},\\ |S|\leq r_k}\E_{\substack{i\in V_k,\\ j\in S_k}}\![d_{i,j}] \quad \text{s.t.} \quad \min_{j\in S_k}d_{i,j}\!\leq\! \delta~~ \forall i\!\in\! V_k.
\end{equation}
% Satisfying the constraint, $\min_{j\in S_k} d_{i,j}~\forall i\in V_k$, in Problem \eqref{eq:subset} requires selecting a large number of elements to ensure that the expected augme $i\in V_k$ is. To be able to select arbitrary small but representative subsets of a given size $r_k$,
Problem \eqref{eq:subset} is NP-hard as it involved calculating the value of objective over an exponential number of subsets.
% , but can be relaxed as follows:
% \begin{equation}
%     S_k^*=\!\!\!\!\argmin_{\substack{S\subseteq V_k},\\ |S|\leq r_k}\sum_{i\in V_k}(\E_{\substack{j\in S_k}}\![d_{i,j}] - \min_{j\in S_k}d_{i,j}).
% \end{equation}
% While a subset can be found by minimizing a weighted combination $\sum_{i\in V_k}(\E_{\substack{j\in S_k}}\![d_{i,j}] - \lambda \min_{j\in S_k}d_{i,j})$
In practice, a diverse subset with small expected augmentation distance to all examples in $V_k$ can be obtained by minimizing the expected augmentation distance between examples in the subset $j\in S_k$ and the rest of examples in the class $V_k\setminus S_k$:\looseness=-1
\begin{equation}\label{eq:subset_relax}
    S_k^*=\!\!\!\!\argmin_{\substack{S\subseteq V_k},\\ |S|\leq r_k}\!\sum_{\substack{i\in V_k\setminus S_k}}\sum_{j\in S_k}d_{i,j}.
\end{equation}
% Problem \eqref{eq:subset_relax} encourages finding a diverse subset that has a small $d_{i,j}$ for all examples in class $k$, by minimizing the expected augmentation distance between $i\in V_k\setminus S_k$, and $j\in S_k$.
The above minimization problem can be turned into maximizing the following monotone submodular\footnote{A set function $F:2^V \rightarrow \mathbb{R}^+$ is \defn{submodular} if $F(e|S)=F(S\cup\{e\}) - F(S) \geq F(T\cup\{e\}) - F(T),$ for any $S\subseteq T \subseteq V$ and $e\in V\setminus T$.  
$F$ is \textit{monotone} if $F(e|S)\geq 0$ for any $e \! \in \! V \! \setminus \! S$ and $S \subseteq V$.} cover problem:
\begin{equation}
    S_k^*=\!\!\!\!\argmax_{\substack{S\subseteq V_k},\\ |S|\leq r_k}\!\sum_{\substack{i\in V_k\setminus S_k}}\sum_{j\in S_k} C-d_{i,j},
\end{equation}
where $C$ is a big constant.  
For maximizing a monotone submodular function, the greedy algorithm provides a $(1-1/e)$ approximation guarantee \citep{wolsey1982analysis}. 
The greedy algorithm starts with the empty set $S_0=\emptyset$, and at each iteration $l$, chooses an element $e\!\in\! V$ such that %the {marginal utility}
$S_l = S_{l-1}\cup\{{\arg\max}_{e\in V} F(e|S_{l-1})\}$. 
The greedy algorithm finds a near-optimal solution of size $r_k$ in $\mathcal{O}(|V|\cdot k)$ time. This complexity can be reduced to $\mathcal{O}(|V|)$ by stochastic evaluation \cite{mirzasoleiman2015lazier} and  accelerated further by lazy evaluations \cite{minoux1978accelerated}.

Intuitively, the above subset contains examples that are highly similar to the other data points in the class $k$.
%%%%
Such examples contain the core features of a class (See Figure \ref{fig:core_features}). As they have a small expected augmentation distance to other examples, they 
produce a large gradient norm and effectively minimize the contrastive loss on the full data. In doing that, they pull together different examples in a class during contrastive learning and let the representations of a class to cluster closely. In addition, as they preserve the class centers, they allow the representations of different classes to be effectively pushed away from each other. \looseness=-1

\begin{figure}
    \centering
    \includegraphics[width=\linewidth, keepaspectratio]{Fig/core_features.png}
    \vspace{-8mm}
    \caption{Core Features}
    \label{fig:core_features}
\end{figure}

%%%%
% Notably, the above objective is non-monotone. That is by adding more examples to the subset $S_k$, the objective may decrease after a while. Intuitively, examples that result in a lower objective are those in low-concentrated regions of a class with a high expected augmentation distance to the rest of the examples. Hence, adding them to the subset increases the error of capturing the class center. \ba{Todo: confirm}

\begin{algorithm}[t]
\caption{Subset Selection for Contrastive SSL}\label{alg}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Budget $B$, Threshold $\tau$
\STATE \textbf{Output:} Subset $S$
\FORALL{$\x \in \X_V$}
    \STATE $score(x) \leftarrow 0$
    \FORALL{$\x' \in \X_V \setminus \{\x\}$}
        \STATE $d_{xx'} = \mathbb{\hat{E}}_{\substack{\x_i \in A(\x) \\ \x'_j \in A(\x')}} \norm{f(x_i) - f(x'_j)}$
        \IF{$d_{xx'} \geq \tau$}
            \STATE $score(x) \leftarrow score(x) + d_{xx'}$
        \ENDIF
    \ENDFOR
\ENDFOR
\STATE $\mathcal{C} = \text{partition of } \X_v \text{ into clusters }$ 
\STATE $S \leftarrow \{\}$
\FORALL{$V_k \in C$}
    \STATE Sort $V_k$ in descending order using $score$
    \STATE $S \leftarrow S \cup V_k[0:\frac{|V_k|}{|\X_V|}\cdot B]$
\ENDFOR 
\STATE \textbf{return} $S$
\end{algorithmic}
\end{algorithm}

% Alternative Lemma: Let $\zeta=\|\muu-\muu_S\|$. Then:
% \begin{align}
%     R^2_{\epsilon}&\!\leq \eta^2(\epsilon) \cdot (\E_{\x\in V_k}\E_{\x_1,\x_2\in A(\x)} \|f(\x_1)-f(\x_2)\|)^2\nonumber\\
%     &\leq\eta^2(\epsilon) \!\cdot \!(\E_{\x\in S_k}\E_{\x_1,\x_2\in A(\x)} \!\|f(\x_1)\!-\!f(\x_2)\|+\zeta \pmb{1})^2 \nonumber\\
%     &\leq\eta^2(\epsilon) \cdot (\LL_{align}(f^S)+\zeta^2\sqrt{d}+2\zeta \muu_S)
% \end{align}
% where $\eta(\epsilon)=\inf_{h\in(0,\frac{\epsilon}{2\sqrt{n}LM})}\frac{4\max \{1,m^2h^{2n}\}}{h^{2n}(\epsilon-2\sqrt{n}LMh)}$. 

% \sj{I think here we can discuss that under some reasonable assumption of how spread out the augmentations of $\x$ are, by virtue of $\x$ being in the main part, we have the equivalent of $d_{\x\x'}$ in data space being small and with lipschitz, we have that the actual $d_{\x\x'}$ is small}. 
% On the other hand, for $\x\in S_k$ we have that, $\max_{\x_1,\x_2\in A(\x)}\|f(\x_1)-f(\x_2)\|\leq \epsilon$ 

% \sj{I think think this holds for most $\x \in S_k$ but not all, so we should maybe include with probability $p$ (large because we minimized alignment loss on subset), this holds.}. 

The following Theorem captures the  required divergence on the centers of the selected examples in every latent class, such that the examples in full data \ba{main part} are classified correctly.
% worst-case difference between the divergence obtained by contrastive learning on the full data vs on the subset 
\begin{theorem}\label{thm:diverge}
Let $V_k^0\subseteq V_k$ be the subset of examples with sharp concentration of augmented data in latent class $k$, i.e., $\sup_{i,j\in V_k^0} \min_{\x\in A(\x_j),\x'\in A(\x_j)}\norm{\x-\x'}\leq \delta$.
Suppose $|V_k^0|\geq \sigma |V_k|$ for $\sigma\in (0,1]$.
% Given a $(\sigma, \delta)$-augmentation used in contrastive SSL and
Assume $\norm{f}= r$, and the subset has $\nu^k_R$ error (Eq. \ref{eq:r_error}) in capturing $R_{\epsilon}(f,V_k)$ and $\nu^k_{\mu}$ error (Eq. \ref{eq:mu_error}) in capturing the center of class $k$. If for any part of classes $l,k\in[K]$ and a constant $C$, %the divergence obtained by contrastive learning on the subset should be larger than 
% the following such that all examples in the main part are classified correctly: \ba{reused r}
the divergence obtained by contrastive learning on the subset is at most
\begin{align}
\frac{r^2C}{p_k}\nu^k_R+2(\max\{\nu^k_{\mu},\nu_{\mu}^l\})^2+4\max\{\nu^k_{\mu},\nu_{\mu}^l\})
% \mathcal{O}(\nu_R+\max\{\nu_k^2,\nu_l^2\}+\max\{\nu_k,\nu_l\})
% \muu_k^S \muu_l^S &<\! r^2 \Big(1-\rho'(\sigma,\gamma,\epsilon,\delta)
%     -\sqrt{2\rho'(\sigma,\gamma,\epsilon,\delta)}-\frac{1}{2}\Delta_\mu' \Big)\nonumber \\ 
%     &+ 2r\zeta_{\max}+\zeta_{\max}^2 \nonumber
\end{align}
larger than the divergence obtained by contrastive learning on the full data, the downstream error rate of NN classifier is \looseness=-1
\begin{equation}
\xi(g_{f^S}(V))\leq (1-\sigma)+R^S_{\epsilon}(V).
\end{equation}

% with $\Delta'_{\mu}= 1 - (\zeta_{max} + \min_k\|\muu^S_k\|) / r^2$, $\rho'(\sigma,\gamma,\epsilon,\delta)=2(1-\sigma)+\frac{R_{\epsilon}+\gamma_1}{p_1}+(\sigma-\frac{R_{\epsilon}+\gamma_1}{p_1})(\frac{L\delta}{r}+\frac{2\epsilon}{r})$. %$\text{ and } \zeta_{max} = max_k[\zeta_k]$

%     {\muu_1^S}^T{\muu_k^S} <\! r^2 (1-\rho_1(\sigma,\delta,\epsilon)-&\sqrt{2\rho_1(\sigma,\delta,\epsilon)}\!-\!\frac{1}{2}\Delta_\mu) \nonumber\\
%     &~+\! 2r\zeta_{\max}\!+\!\zeta_{\max}^2 \nonumber
% \end{align}
% \begin{align}
%     \|{\muu_l^S}^T{\muu_k^S}-\muu_l^T\muu_k\| \!<\! 
%     \phi(\gamma)\!-\!\sqrt{\phi(\gamma)}\!+\! 2r{\max}(\zeta_l,\zeta_k)\!+\!\zeta_{l}\zeta_k, \nonumber
% \end{align}
% for any pair of $(l, k)$ with $l\!\neq \!k$, where $\phi(\gamma)\!=\!\frac{\gamma}{p_k}(1\!+\!\frac{L\delta}{r}\!-\!\frac{2\epsilon}{r})$. %and the downstream error rate of NN classifier $g_f$ is $\xi(g_f) \leq (1 - \sigma) + R_{\epsilon}$.
% where $\rho{\max}(\sigma,\delta,\epsilon)=2(1-\sigma)+\frac{R_{\epsilon}}{\min_l p_l} +\sigma (\frac{L\delta}{r} + \frac{2\epsilon}{r})$ and $\Delta_{\mu}=1-\min_{k\in[K]}\|\muu_k\|^2 /r^2$.
\end{theorem}
Theorem \ref{thm:diverge} shows that if the subset captures the class centers and alignment closely (i.e. $\nu_R$ and $\nu_{\mu}$ are small), then minimizing the contrastive loss results in the same downstream generalization performance for the linear classifier. 
Note that minimizing the contrastive loss on the subset can potentially separate the class means better than contrastive learning on full data, as the subset does not include many points in the low-concentrated areas. In this case, contrastive learning on a large enough subset can achieve a comparable or even superior downstream performance than contrastive learning on the full data. \ba{Todo: confirm experimentally} 
% \begin{corollary}
% For a $L$-Lipschitz continuous encoder $f$ with norm 1 trained on the subset, if 
% \begin{align}
%     %\muu_k^T\muu_l&<
%     &\log(\exp\{\frac{\LL_2(f)+\tau(\sigma,\delta,\epsilon,R_{\epsilon})}{p_k p_l}\}-\exp(1-\epsilon)\nonumber \\
%     &<\! r^2 (1\!-\!\rho'_1(\sigma,\delta,\epsilon,\gamma)\!-\!\sqrt{2\rho'_1(\sigma,\delta,\epsilon,\gamma)}\!-\!\frac{1}{2}\Delta'_\mu)\nonumber \\ 
%     &+ 2r\zeta_{\max}+\zeta_{\max}^2
% \end{align}
% the generalization ability of encoder $f$ on the downstream task is 
% \begin{equation}
%     \zeta(g_f) \leq (1 - \sigma) + \eta(\epsilon) R_\epsilon.
% \end{equation}
% \end{corollary}
% \sj{thm1 - alignment preserved}
% $L_{align}$ on subset makes  $L_{align}$ on full set small. 
 
%  \sj{Thm2 - divergence between class centers preserved}
% objective on subset ensures that means do not change. 

 % \sj{Corollary generalization good} Means don't change \textbf{thm2} and $S_\epsilon \cap \text{main part}$ doesn't change \textbf{thm1}, so generalization good by invoking \textbf{iclr thm1}


%%%%%%%%%%%%%%%

\section{Finding the Subset}
Next, we discuss how we can solve Problem \eqref{eq:subset} to find the most effective subsets for contrastive SSL.
We first discuss finding expected augmentation distance, and then explain how we can find a subset from each class. 

\subsection{Estimating Expected Augmentation Distance}
To estimate the expected augmentation distances $d_{\x,\x}$, %between data points $\x$ and $\x'$, 
we uniformly sample pairs of augmented views of $\x$ and $\x'$, i.e., $(\x_a, \x'_a)$ where $\x_a \!\in\! A(\x), \x'_a \!\in\! A(\x')$, and $A(.)$ is the set of discrete and continuous transformations. 
In particular, we use random crop, random resizing, random horizontal flips and color distortion, as the set of transformations used in \cite{cl_simclr}.
Then the pairwise expected augmentation distance is calculated for all $\x, \x' \in V_k$, according to Eq. \eqref{eq:dist}. In our experiments, we show that the distances can be calculated using the embeddings of a partially-trained network or a smaller fully-trained network. \ba{Todo: experiments on early, smaller net, num augs} \sj{discuss threshold} \ba{either here or in experiments}


\subsection{Finding the Latent Classes}
Next, we discuss how to find examples in every class $V_k$. If we had the labels, we would know exactly which examples are in a class $V_k$ and we could find a subset from each class separately. Without the labels, we need to first partition the data into $k$ classes. We investigate two different ways to approximately find examples in each class. In the first approach, we find different classes by clustering the representations of a network that is fully trained with contrastive SSL. \ba{Todo: early/transfer?}
Note that, we do not require to know the exact number of classes to find the same number of clusters. As we show in our experiments, finding a larger number of clusters than the number of labels in the downstream task does not harm the performance. \ba{Todo}
Hence, one can always find a relatively large number of clusters and find a subset from each of the finer-grained clusters.
In the second approach, we consider the case where a small subset of labels of the downstream task is available. We show that as small as 1\% of the labels of the downstream task is enough to use a proxy model such as CLIP \cite{radford2021learning} to approximately find the examples in every class.
In both cases, we find a subset $S_k$ from each class by solving the minimization Problem \eqref{eq:subset}.
\ba{we don't need to know the class, subclass works as well (since things are linearly separable)}.


The pseudocode is illustrated in Alg. \ref{alg}.


